Stackelberg Vertex Cover on a Path

A Stackelberg Vertex Cover game is played on an undirected graph $\mathcal{G}$ where some of the vertices are under the control of a \emph{leader}. The remaining vertices are assigned a fixed weight. The game is played in two stages. First, the leader chooses prices for the vertices under her control. Afterward, the second player, called \emph{follower}, selects a min weight vertex cover in the resulting weighted graph. That is, the follower selects a subset of vertices $C^*$ such that every edge has at least one endpoint in $C^*$ of minimum weight w.r.t.\ to the fixed weights, and the prices set by the leader. Stackelberg Vertex Cover (StackVC) describes the leader's optimization problem to select prices in the first stage of the game so as to maximize her revenue, which is the cumulative price of all her (priceable) vertices that are contained in the follower's solution. Previous research showed that StackVC is \textsf{NP}-hard on bipartite graphs, but solvable in polynomial time in the special case of bipartite graphs, where all priceable vertices belong to the same side of the bipartition. In this paper, we investigate StackVC on paths and present a dynamic program with linear time and space complexity.

==> TikzSet.tex <==
\makeatletter
\tikzset{
	circle split part fill/.style  args={#1,#2}{%
		alias=tmp@name,
		postaction={%
			insert path={
				\pgfextra{% 
					\pgfpointdiff{\pgfpointanchor{\pgf@node@name}{center}}%
					{\pgfpointanchor{\pgf@node@name}{east}}%            
					\pgfmathsetmacro\insiderad{\pgf@x}
					%\begin{scope}[on background layer]
					%\fill[#1] (\pgf@node@name.base) ([xshift=-\pgflinewidth]\pgf@node@name.east) arc
					%                    (0:180:\insiderad-0.5\pgflinewidth)--cycle;
					%\fill[#2] (\pgf@node@name.base) ([xshift=\pgflinewidth]\pgf@node@name.west)  arc
					%                     (180:360:\insiderad-0.5\pgflinewidth)--cycle;  
					\fill[#1] (\pgf@node@name.base) ([xshift=-\pgflinewidth]\pgf@node@name.east) arc
					(0:180:\insiderad-\pgflinewidth)--cycle;
					\fill[#2] (\pgf@node@name.base) ([xshift=\pgflinewidth]\pgf@node@name.west)  arc
					(180:360:\insiderad-\pgflinewidth)--cycle;  
	}}}},
	rectangle split part fill/.style  args={#1,#2}{%
		alias=tmp@name,
		postaction={%
			insert path={
				\pgfextra{% 
					\pgfpointdiff{\pgfpointanchor{\pgf@node@name}{center}}%
					{\pgfpointanchor{\pgf@node@name}{east}}%            
					\pgfmathsetmacro\insiderad{\pgf@x}
					%\begin{scope}[on background layer]
					%\fill[#1] (\pgf@node@name.base) ([xshift=-\pgflinewidth]\pgf@node@name.east) arc
					%                    (0:180:\insiderad-0.5\pgflinewidth)--cycle;
					%\fill[#2] (\pgf@node@name.base) ([xshift=\pgflinewidth]\pgf@node@name.west)  arc
					%                     (180:360:\insiderad-0.5\pgflinewidth)--cycle;  
					\fill[#1] (\pgf@node@name.west) -- (\pgf@node@name.north west) -- (\pgf@node@name.north east) -- (\pgf@node@name.east) -- (\pgf@node@name.west);
					\fill[#2] (\pgf@node@name.west) -- (\pgf@node@name.south west) -- (\pgf@node@name.south east) -- (\pgf@node@name.east) -- (\pgf@node@name.west); 
					\draw[thick] (\pgf@node@name.north west) -- (\pgf@node@name.south west) -- (\pgf@node@name.south east) -- (\pgf@node@name.north east) -- (\pgf@node@name.north west) -- (\pgf@node@name.south west); 
	}}}},
}  
\makeatother  
%
%\newlength{\kandinsky} %defines a new length 
%\settowidth{\kandinsky}{\footnotesize Wassily Kandinsky} 
%set new length for the proper parbox width
\makeatletter
\tikzset{
	every node/.style={
		%thick,
		%circle,
		inner sep = 0pt,
		outer sep = 0pt,
		minimum size = .7cm,
		draw,
		text = white,
		%line width=1mm,
	},
	plain/.style={
		draw = none,
		fill = none,
		minimum size = .6cm
	},
	aPartition/.style={
		%fill = graphcolorpeach-orange,
		shape = rectangle,
	},
	bPartition/.style={
		%fill = graphcolorpeach,
		shape = circle
	},
	background/.style={
		opacity=.40,
		fill = gray,       
	},
	cover/.style={
		fill = RWTH_Magenta,
		text = white
	},
%	priceable/.style={
%		fill = RWTH_Magenta,
%		text = white,
%		%very thick,
%	},
%	fixed price/.style={
%		fill = HKS44,
%		text = white,
%		very thick,
%	},
	CoreCoverA/.style={
		rectangle split part fill={RWTH_Magenta, HKS44},
		text = white,
	},
	CoreCoverB/.style={
		circle split part fill={RWTH_Magenta, HKS44},
		text = white,
	},
	CoreComplementA/.style={
		rectangle split part fill={HKS44_25prcnt, HKS44},
		text = white,
	},
	CoreComplementB/.style={
		circle split part fill={HKS44_25prcnt, HKS44},
		text = white,
	},
%	priceable CoverB/.style={
%		%circle split part fill={RWTH_Magenta, HKS44},  
%		circle split part fill={RWTH_Magenta, RWTH_Lightblue}, 
%		text = white,
%		thick,	
%	},
%	fixed price CoverA/.style={
%		%circle split part fill={RWTH_Magenta, HKS44},  
%		rectangle split part fill={HKS44, RWTH_Lightblue}, 
%		text = white,
%		thick,	
%	},
%	fixed price CoverB/.style={
%		%circle split part fill={RWTH_Magenta, HKS44},  
%		circle split part fill={HKS44, RWTH_Lightblue}, 
%		text = white,
%		thick,	
%	},
	blue/.style={
		fill = HKS44,
		text = white
	},
	light blue/.style={
		fill = HKS44_25prcnt,
		text = white
	},
	magenta/.style={
		fill = RWTH_Magenta,
		text = white
	},
	complementEdge/.style={
		dashed,
		color = black
	},
	backgroundEdge/.style={
		opacity = .5,
		dashed
	},
	textbox/.style={
		shape = rectangle,
		draw = none,
		minimum height=\textboxHeight,
		inner ysep = 0cm,
		inner xsep = .1cm,
		outer sep = 0cm,
	},
	vertex/.style={
		inner sep = 0cm,
		outer sep = 0cm,
		minimum size=.85cm,
		draw
	}
}
\makeatother 

\newlength{\textboxHeight} %defines a new length 
\setlength{\textboxHeight}{.53cm}
\newlength{\vertSpacing} %defines a new length 
\setlength{\vertSpacing}{.5cm}
\newlength{\fullVertSpacing}
\setlength{\fullVertSpacing}{\vertSpacing}
\addtolength{\fullVertSpacing}{\vertSpacing}
\addtolength{\fullVertSpacing}{\textboxHeight}

==> graphics/Branching-MonotonousCase.tex <==
\tikzset{
	every node/.style={
		thick,
		inner xsep = 3pt,
		inner ysep = 2pt,
		% minimum size = 1cm,
		text = black,
		font = {\bfseries\small},
		%draw
		%line width=1mm,
	},
}
\begin{figure}[tbph]
	\resizebox{\textwidth}{!}{
		\centering
		\begin{tikzpicture}
			\centering
			\node[rectangle, textbox] (AGR20) {$\AGR{2}{i \Shortminus 2}$};
			%\node[above = \vertSpacing of O11, shape = rectangle, draw, fill = none, minimum size=.85cm, inner sep=1.5pt](p0){\normalsize $p_{i-2}$}; 
			\node[above = \fullVertSpacing of AGR20, anchor = south, vertex, draw = none](d0){\tikzdots};
			\node[below = 1.3cm of AGR20, outer sep = 0, shape = rectangle, minimum width= .7cm, minimum height= 0cm](h0){};
			%%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%%
			\node[right = 1cm of AGR20.east, textbox](O21){\color{RWTH_Magenta}$\Option_2[i \Shortminus 1]$};
			\node[above = \vertSpacing of O21.north, anchor=south, textbox](O11){\color{HKS44}$\Option_1[i \Shortminus 1]$};
			\node[below = \vertSpacing of O21.south, anchor=north, textbox](O31){\color{RWTH_Orange}$\Option_3[i \Shortminus 1]$};
			%
			\node[above = \vertSpacing of O11.north, anchor = south, vertex](p1){\normalsize $p_{i-1}$}; 
			%%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%%
			\node[right= 1cm of O21, textbox](AGR11){$\AGR{1}{i \Shortminus 1}$};
			\node[right = 2.7cm of p1, vertex, draw = none](d1){\tikzdots};
			\node[right= \vertSpacing of AGR11.east, anchor=west](AGR21){$\AGR{2}{i \Shortminus 1}$};
			%
			\node[right = .75cm of AGR21, textbox](O22){\color{RWTH_Magenta}$\Option_2[i]$};
			%\node[above = \vertSpacing of O22, textbox](O12){\color{HKS44}$\Option_1[i]$};
			\node[opacity=0, above = \vertSpacing of O22, textbox](O12){\color{HKS44}$\Option_1[i]$}; % INVISIBLE!
			%\node[below = \vertSpacing of O22, textbox](O32){\color{RWTH_Orange}$\Option_3[i]$};
			%
			\node[above = \vertSpacing of O12.north, anchor = south, vertex, shape = circle](p2){\normalsize $p_{i}$};
			%%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%%
			%\node[right= 1cm of O22, textbox](AGR12){$\AGR{1}{i}$};
			\node[right = 1.45cm of p2, vertex, draw = none](d2){\tikzdots};
			%
			\node[right= .75cm of O22, textbox](AGR22){$\AGR{2}{i}$};
			%
			\node[right = 1cm of AGR22, textbox](O23){\color{RWTH_Magenta}$\Option_2[i \Shortplus 1]$};
			\node[above = \vertSpacing of O23, textbox](O13){\color{HKS44}$\Option_1[i \Shortplus 1]$};
			\node[below = \vertSpacing of O23, textbox](O33){\color{RWTH_Orange}$\Option_3[i \Shortplus 1]$};
			%
			\node[above = \vertSpacing of O13.north, shape = circle, vertex](p3){\normalsize $p_{i+1}$};
			%%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%%
			\node[right= 1cm of O23, textbox](AGR13){$\AGR{1}{i \Shortminus 1}$};
			\node[right= 1.55cm of p3, vertex, draw = none](d3){\tikzdots};
			\node[right= 1.55cm of d3, vertex](p4){$p_{i+2}$};
			\node[right= 1cm of AGR13.east, outer ysep=.1cm](AGR23){\tikzdots};
			\node[below = 1.8cm of AGR23, outer sep = 0, shape = rectangle, minimum width= .7cm, minimum height= 0cm, outer ysep=.1cm](h4){\tikzdots};
			%%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%%
			%%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%%
			%%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%%
			\draw[-stealth, bend right, out=-30, in=-150] (h0.north west) to (AGR21);
			%
			\draw[-stealth] (AGR20.north east) to (O11.south west);
			\draw[-stealth] (AGR20.east) to (O21.west);
			\draw[-stealth] (AGR20.south east) to (O31.north west);
			%
			\draw[-stealth] (O11.south east) to (AGR11.north west);
			\draw[-stealth] (O21.east) to (AGR11.west);
			%\draw[-stealth] (O31.north east) to (AGR11.south west);
			\draw[-stealth, bend right, out=-30, in=-140] (O31.east) to (AGR22);
			%
			\draw[-stealth] (AGR11) to (AGR21);
			\draw[-] (d0) to (p1);
			\draw[-] (p1) to (d1);
			%%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%%
			%\draw[-stealth] (AGR21.north east) to (O12.south west);
			\draw[-stealth] (AGR21.east) to (O22.west);
			%\draw[-stealth] (AGR21.south east) to (O32.north west);
			%
			%\draw[-stealth] (O12.south east) to (AGR12.north west);
			\draw[-stealth] (O22.east) to (AGR22.west);
			%\draw[-stealth] (O32.north east) to (AGR12.south west);
			%\draw[-stealth, bend right, out=-20, in=-140] (O32.east) to (AGR23);
			%
			%\draw[-stealth] (AGR12) to (AGR22);
			\draw[-] (d1) to (p2);
			\draw[-] (p2) to (d2);
			%%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%% %%%
			\draw[-stealth] (AGR22.north east) to (O13.south west);
			\draw[-stealth] (AGR22.east) to (O23.west);
			\draw[-stealth] (AGR22.south east) to (O33.north west);
			%
			\draw[-stealth] (O13.south east) to (AGR13.north west);
			\draw[-stealth] (O23.east) to (AGR13.west);
			%\draw[-stealth] (O33.north east) to (AGR13.south west);
			%
			\draw[-stealth] (AGR13) to (AGR23);
			\draw[-] (d2) to (p3);
			\draw[-] (p3) to (d3);
			\draw[-] (d3) to (p4);
			\draw[-stealth, out=-20, in=170] (O33.east) to (h4);
		\end{tikzpicture}
	}
	\caption{A sequence of alternating priceable vertices interrupted by two consecutive priceable vertices from the same side of the bipartition.}
	\label{fig:Branching-MonotonousCase}
\end{figure}

